QuadraNet V2: Efficient and Sustainable Training of High-Order Neural Networks with Quadratic Adaptation

Machine learning is evolving towards high-order models that necessitate pre-training on extensive datasets, a process associated with significant overheads. Traditional models, despite having pre-trained weights, are becoming obsolete due to architectural differences that obstruct the effective transfer and initialization of these weights. To address these challenges, we introduce a novel framework, QuadraNet V2, which leverages quadratic neural networks to create efficient and sustainable high-order learning models. Our method initializes the primary term of the quadratic neuron using a standard neural network, while the quadratic term is employed to adaptively enhance the learning of data non-linearity or shifts. This integration of pre-trained primary terms with quadratic terms, which possess advanced modeling capabilities, significantly augments the information characterization capacity of the high-order network. By utilizing existing pre-trained weights, QuadraNet V2 reduces the required GPU hours for training by 90\% to 98.4\% compared to training from scratch, demonstrating both efficiency and effectiveness.

==> _txt/_hist/1_Introduction.tex <==
\section{Introduction}
\begin{comment}
The applications of deep learning models towards downstream tasks usually follow the procedure that pre-training a model with large scale data and fine-tuning the model to the specific task dataset. 
   % However, as the emerge of large-language model~\cite{brown2020language,touvron2023llama} and contrastive language-image pretraining~\cite{radford2021learning} put the training data scale towards web-wide, 
   However, in the era of large foundation model~\cite{brown2020language,touvron2023llama,radford2021learning}, the web-wide scale dataset has pushed the size of deep neural network model's to the level  of billions of parameters, for example, the ConvNext V2~\cite{liu2022convnet} and Swin Transformer V2~\cite{liu2022swin} have achieved more the 3 Billion parameters benefit from novel training scheme. 
        Transfer learning based model full fine-tuning in such scale becomes unacceptable in terms of cost.    
            Some attempted to lessen this issue by tuning select parameters~\cite{shen2021partial} or acquiring supplementary adapter~\cite{hu2021lora} to address novel tasks. 
        In adapter way, we can easily freeze the large pre-trained model and only update and store a light adapter with few task-specific parameters.
\end{comment}
Deep learning models are commonly applied to downstream tasks by first pre-training them on large-scale datasets and then fine-tuning them on specific task datasets. However, with the emergence of large foundation models such as those introduced by \cite{brown2020language, touvron2023llama, radford2021learning}, the scale of web-wide datasets has led to deep neural network models reaching billions of parameters. For instance, models like ConvNext V2 \cite{liu2022convnet} and Swin Transformer V2 \cite{liu2022swin} have exceeded 3 billion parameters, benefiting from innovative training approaches. Transfer learning-based full fine-tuning  models at such a massive scale has become impractical due to the associated costs. Some researchers have attempted to address this issue by adjusting specific parameters \cite{shen2021partial} or integrating supplementary adapters \cite{hu2021lora} to tackle novel tasks. With the adapter approach, the large pre-trained model can be frozen, and only a lightweight adapter with a few task-specific parameters needs to be updated and stored. In this plug and play mode, the cost of adapting a large model is greatly reduced and the lifelong learning capacity of the model is improved.

However, traditional adapters typically model the distribution shift between pretraining task data and downstream task data in a simplistic linear format, assuming a straightforward relationship between the two datasets. 
    This oversimplified approach may fail to capture the nuanced and non-linear nature of the actual shift as show in Fig~\ref{fig:shift}, potentially leading to suboptimal performance in adapting to the downstream task.
        Introducing a high-order adapting approach can potentially address the aforementioned issue. However, designing such a high-order adapter faces two primary challenges: Firstly, higher-order computations often entail a quadratic or even higher-dimensional parameter space. Secondly, while confining the approach to a polynomial space, even with a high degree, the representational dimensionality remains severely limited. This constraint poses difficulties in ensuring the separability of high-dimensional non-linear states.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{_fig/newToyCase0.pdf}
  \caption{Non-Linear Distribution Shift}
  \label{fig:shift}
  \vspace{-3mm}
\end{figure}

In addressing the first challenge, we stumbled upon a remarkable revelation: the quadratic component embedded within QuadraNet~\cite{xu2023quadranet} can seamlessly double as a conventional convolutional neural network adapter. This unexpected synergy allows for the incorporation of high-order features into the adaptation process with astonishing efficiency, requiring only marginal supplementary computational resources. This phenomenon arises from the structural similarity between the quadratic term in QuadraNet and a typical adapter. Remarkably, when the quadratic term is removed, QuadraNet aligns structurally with a ConvNext model.
    The difference between training a QuadraNet model and utilizing the quadratic term as an adapter for tuning a ConvNext model resides in their procedural approaches. When training a QuadraNet, the model undergoes full-fledged training from the scratch, starting with random initialization and learning all parameters through the training process. In contrast, when employing the quadratic term as an adapter for fine-tuning a ConvNext model, the process entails an initial phase where only the primary components of the ConvNext model are trained. Subsequently, the trained ConvNext model is adapted by incorporating the quadratic term.

Regarding the second challenge, we reveals that the computation of quadratic terms bears a striking resemblance to conducting inner product calculations. It's noteworthy that in Support Vector Machines (SVM), the kernel method serves as a common strategy for transforming data into a higher-dimensional space to compute its non-linear representation features, allowing models to effectively capture complex relationships between data points that may not be discernible in the original input space.

In this paper, we present QuadraNet V2, an innovative approach that harnesses quadratic kernel adapters to train quadratic neural networks. By incorporating these adapters, our method adeptly captures the nuanced data shift between the original pre-training data and the downstream task data. Consequently, this modeling strategy leads to a substantial improvement in the model's performance on the target dataset, demonstrating its efficacy in addressing the challenges posed by distribution shift in deep learning tasks. Compared with vanilla QuadraNet~\cite{xu2023quadranet}, QuadraNet V2 showcases remarkable advancements, not only in its fundamental model performance but also in its effectiveness across a spectrum of downstream tasks such as object detection and semantic segmentation. Our experiments show the great efficiency of quadratic adapter and the performance gain benefit from powerful representation capacity of kernel enhanced quadratic adapters. 

\textbf{Contributions.} We make the following contributions:
\begin{itemize}
    \item We shed light on the critical aspect of considering the high-order relation when modeling the distribution shift between pre-training data and task data.
    \item We introduce a novel approach by proposing the utilization of the quadratic term of vanilla quadratic neural networks as an adapter for adapting deep models in a high-order fashion. 
    \item We advance the methodology by advocating for the integration of the kernel method to expand the representation space of quadratic adapter. By leveraging this technique, we effectively explore and capture more complex nonlinear relations within the data, leading to improved model generalization.
\end{itemize}

%强调一下从头开始的quadratic NN预训练将耗费大量成本。

%写到第3栏中到结束的位置

==> _txt/_hist/1_Introduction_new.tex <==
\section{Introduction}
% The current trend in neural network development is towards high-order neural networks with strong representational properties. Such higher-order neural networks are represented by ViT, HorNet, and QuadraNet. These models have shown strong performance in vision, language, speech, etc. However, the inherent problem of such high-order neural networks is that when scaling to larger scale, each new model has to be built by restarting the training on a large-scale dataset, which implies a huge computational scale. As an example, a typical QuadraNet-B model pre-trained on ImageNet-21k medium scale will spend tens of thousands of GPU hours on A100 for each training from scratch, implying nearly $20,000 in computational expense (April 2024 computing power prices).
The evolving landscape of neural network development is increasingly characterized by the adoption of high-order architectures, which possess robust representational capacities. Prominent examples of such architectures such as ViT~\cite{dosovitskiy2020image} MogaNet~\cite{li2024moganet} and HorNet~\cite{rao2022hornet} which have demonstrated exceptional performance across various domains such as vision, language processing, and speech recognition. Despite their strengths, a critical limitation of these high-order neural networks is the necessity to reinitiate training from scratch for each new model iteration, particularly when scaling up. This approach requires training on large-scale datasets, which results in substantial computational demands. For instance, training a typical HorNet-B model on the medium-scale ImageNet-21k dataset can consume around 8000 GPU hours on NVIDIA's A100 GPUs, translating to an approximate computational cost of nearly \$20,000 today. 
%This situation is exacerbated by the web-wide data training that is popular today, where a new high-order large model training is expected to cost hundreds of thousands or even millions of dollars. 
This necessitates a reconsideration of model scalability and efficient training in neural network development strategies.


%Meanwhile, the machine learning community has now trained a very large number of conventional neural networks, such as convolutional neural networks, with super-sized data. The gradual phasing out of these neural networks in the trend towards higher-order models means that these model weights, which have been trained at great cost, will be discarded.
A pressing challenge in this transition is the difficulty of repurposing existing pre-trained weights to construct powerful high-order models.
As the machine learning community increasingly gravitates towards high-order neural network architectures, there is a noticeable departure from conventional models such as convolutional neural networks (CNNs), which have been extensively trained on super-sized datasets. This shift implies that the substantial investments in training these traditional networks may soon become obsolete as their relevance wanes. Consequently, the model weights, developed at significant computational and financial costs, risk being discarded as these models are phased out. This raises significant concerns about the sustainability and resource efficiency of current machine learning practices.

The core of this issue lies in the substantial architectural disparities between traditional and high-order networks, which hinder the efficient transfer and utilization of these pre-trained weights for effective model initialization. 


Analyzing the aforementioned challenges, we propose that the framework for developing high-order neural networks should emphasize sustainability. Specifically, this entails two key objectives: (1) constructing new high-order networks with minimal training requirements, and (2) harnessing the value of existing pre-trained weights. To achieve these goals, high-order models should be designed to be structurally adaptable, capable of conforming to diverse architectural designs. Furthermore, these advanced models should exhibit robust expressive capabilities and strong transfer learning performance. Importantly, such models should not only achieve high performance ceilings but also possess the ability to directly leverage knowledge from pre-existing models.


    We note that the quadratic neuron can be decomposed into two parts, a primary term that can be given weight by the primary neuron, and a quadratic term with strong representational and migration capabilities. 
        And the two parts of the quadratic neuron can be trained separately.
    This gives the opportunity to utilize existing large-scale pre-trained weights to build a high-order neural network with quadratic term adaptation.
    
In this paper, we propose a framework for building such efficient and sustainable high-order learning using quadratic neural networks. We propose a method to initialize the primary term of the quadratic neuron using an ordinary neural network, and then use the quadratic term to further learn the non-linearity of the data or data shift as an adaptation. 
     To achieve more efficient high-order neural interaction, we further made the following optimizations to the quadratic neurons.
        We first make a rank decomposition of the quadratic term of the quadratic neuron to reduce its computational complexity from squared complexity to linear complexity; we incorporate a null design in the quadratic term to sparsify its high-order interactions and capture the offset between the pre-training data and the tuning data through fewer interactions; and we incorporate a kernel method design to make the high-order interactions themselves characterization performance is stronger.

Following such a framework, in this paper, we build a new family of high-order neural networks--CodeName, as an case study. We first use the existing large-scale pre-trained ConvNeXt to initialize the model's primary term. Then, we train the model's secondary adaptation term during the training phase to enable the model to efficiently model the offset between the pre-trained data and the downstream task data. Our experiments demonstrate the excellent performance of CodeName on various tasks. At the same time, our experimental results show that the GPU hours required to train the model to the same accuracy as training from scratch are reduced by ~90\% to 98.4\% by utilizing the existing pre-trained weights in the training approach.

Our contributions are:





==> _txt/_hist/2_RelatedWork.tex <==

\section{Related Works}
\subsection{Neural Network Adapter}
\subsection{Kernel Method in Neural Networks}
\subsection{Quadratic Neural Networks}

%写到第4栏尾部或者第5栏中部结束
